Stochastic Bridges as Effective Regularizers for Parameter-Efficient Tuning

Parameter-efficient tuning methods (PETs) have achieved promising results in tuning large pre-trained language models (PLMs). By formalizing frozen PLMs and additional tunable parameters as systems and controls respectively, PETs can be theoretically grounded to optimal control and further viewed as optimizing the terminal cost and running cost in the optimal control literature. Despite the elegance of this theoretical grounding, in practice, existing PETs often ignore the running cost and only optimize the terminal cost, i.e., focus on optimizing the loss function of the output state, regardless of the running cost that depends on the intermediate states. Since it is non-trivial to directly model the intermediate states and design a running cost function, we propose to use latent stochastic bridges to regularize the intermediate states and use the regularization as the running cost of PETs. As the first work to propose regularized PETs that use stochastic bridges as the regularizers (running costs) for the intermediate states, we show the effectiveness and generality of this regularization across different tasks, PLMs and PETs. In view of the great potential and capacity, we believe more sophisticated regularizers can be designed for PETs and better performance can be achieved in the future. The code is released at \url{https://github.com/thunlp/stochastic-bridge-pet/tree/main}.

==> tables/centroid_correlation.tex <==
% \begin{wraptable}{r}{4.8cm}
\begin{table}
    \centering
    \renewcommand{\arraystretch}{0.9}
    \begin{tabular}{l r@{}l r@{}l}
        \toprule
        %  & \multicolumn{4}{c}{Coef.} \\
        % \cmidrule(lr){2-5}
        Dataset & \multicolumn{2}{c}{\textsc{PDF}} & \multicolumn{2}{c}{\textsc{SDE}}\\
        \midrule
        MNLI & 0&.928$^{***}$ & 0&.894$^{***}$ \\
        QQP & 0&.715$^{*}$ & 0&.897$^{***}$ \\
        QNLI & 0&.971$^{***}$ & 0&.837$^{**}$ \\
        SST-2 & 0&.966$^{***}$ & 0&.867$^{***}$ \\
        MRPC & 0&.226 & 0&.433 \\
        CoLA & 0&.633$^{*}$ & 0&.807$^{**}$ \\
        RTE & 0&.440 & 0&.589$^{*}$ \\
    \bottomrule
    \end{tabular}
    \caption{Pearson's correlation between the regularization strength $\alpha$ and the average distance between the centroids of different label clusters. $^{***}$: $\mathit{p}<.001$,  $^{**}$: $\mathit{p}<.01$, $^{*}$: $\mathit{p}<.05$.}
    \label{tab:centroid-correlation}
    \vspace{-1em}
\end{table}

==> tables/deberta_32shot.tex <==
\begin{table}[t!]
    \centering
    \caption{The results on GLUE for $\deberta$ under 16-shot setting.}
    \setlength{\tabcolsep}{4pt}
    \begin{tabular}{l *{9}{r}}
    \toprule
         PET & MNLI & QQP & QNLI & SST-2 & MRPC & CoLA & RTE & Average & $\Delta$\\ 
    \midrule
        \textsc{Prompt} & 34.4$_{1.2}$ & 53.2$_{5.1}$ & 51.7$_{1.7}$ & 73.3$_{8.7}$ & 50.2$_{3.2}$ & 2.5$_{2.5}$ & 52.2$_{4.9}$ & 45.4$_{2.1}$ &-\\
        \textsc{+Brown\_PDF} & \textbf{36.5}$_{2.1}$ & \textbf{62.5}$_{5.2}$ & 54.9$_{3.6}$ & \textbf{91.8}$_{0.8}$ & 56.3$_{2.5}$ & \textbf{9.6}$_{10.3}$ & \textbf{54.9}$_{3.0}$ & \textbf{52.4}$_{2.2}$ & \textbf{7.0}\\ 
        \textsc{+Brown\_SDE} & 36.1$_{0.9}$ & 61.8$_{1.9}$ & \textbf{58.4}$_{8.1}$ & 89.4$_{1.1}$ & \textbf{56.4}$_{4.2}$ & 7.8$_{6.3}$ & 53.9$_{2.1}$ & 52.0$_{1.2}$ &6.6\\
    \midrule
        \textsc{LoRA} & 53.9$_{3.2}$ & 71.8$_{3.0}$ & 71.3$_{2.3}$ & \textbf{93.1}$_{0.8}$ & \textbf{63.7}$_{2.9}$ & 11.3$_{2.4}$ & 59.9$_{2.9}$ & 60.7$_{0.7}$ &-\\
        \textsc{+Brown\_PDF} & \textbf{62.7}$_{3.3}$ & 73.1$_{0.8}$ & 77.5$_{4.5}$ & \textbf{93.1}$_{0.8}$ & 63.3$_{2.1}$ & 25.5$_{11.4}$ & \textbf{64.6}$_{5.8}$ & 65.7$_{1.0}$ &5.0\\
        \textsc{+Brown\_SDE} & 60.4$_{4.2}$ & \textbf{74.6}$_{2.2}$ & \textbf{79.8}$_{2.5}$ & 92.0$_{2.0}$ & 62.9$_{4.7}$ & \textbf{39.4}$_{9.7}$ & 64.3$_{5.5}$ & \textbf{67.6}$_{1.9}$ & \textbf{6.9}\\ 
    \midrule
        \textsc{BitFit} & 46.7$_{2.3}$ & 72.1$_{0.8}$ & 68.3$_{4.3}$ & \textbf{92.1}$_{0.7}$ & 58.1$_{2.8}$ & 13.2$_{4.8}$ & 59.4$_{0.6}$ & 58.6$_{1.1}$ &-\\
        \textsc{+Brown\_PDF} & 50.2$_{2.2}$ & \textbf{73.5}$_{0.6}$ & 74.9$_{4.6}$ & 91.4$_{0.8}$ & 57.5$_{2.5}$ & 14.5$_{4.2}$ & 61.4$_{2.5}$ & 60.5$_{0.7}$ &1.9\\
        \textsc{+Brown\_SDE} & \textbf{51.1}$_{2.3}$ & 72.9$_{1.4}$ & \textbf{77.7}$_{2.2}$ & 89.8$_{1.3}$ & \textbf{60.2}$_{3.8}$ & \textbf{32.2}$_{10.8}$ & \textbf{62.6}$_{5.7}$ & \textbf{63.8}$_{1.9}$ & \textbf{5.2}\\ 
    \midrule
        \textsc{Adapter} & 53.1$_{5.3}$ & 72.9$_{1.7}$ & 71.5$_{4.3}$ & 92.2$_{1.0}$ & 62.3$_{1.8}$ & 15.3$_{6.2}$ & 59.4$_{4.8}$ & 61.0$_{1.7}$ &-\\
        \textsc{+Brown\_PDF} & \textbf{60.2}$_{4.7}$ & 74.5$_{1.0}$ & \textbf{79.7}$_{1.9}$ & \textbf{92.3}$_{0.4}$ & 63.3$_{3.5}$ & 23.6$_{13.2}$ & 64.0$_{1.8}$ & 65.4$_{0.9}$ &4.4\\
        \textsc{+Brown\_SDE} & 60.0$_{3.1}$ & \textbf{75.2}$_{1.1}$ & 79.4$_{2.5}$ & \textbf{92.3}$_{0.8}$ & \textbf{65.3}$_{4.3}$ & \textbf{38.3}$_{6.3}$ & \textbf{64.3}$_{1.9}$ & \textbf{67.8}$_{1.4}$ & \textbf{6.8}\\ 
    \bottomrule
    \end{tabular}
    \label{tab:glue-deberta-16shot}
\end{table}


==> tables/deberta_4shot.tex <==
\begin{table}[t!]
    \centering
    \caption{The results on GLUE for $\deberta$ under 4-shot setting.}
    \setlength{\tabcolsep}{4pt}
    \begin{tabular}{l *{9}{r}}
    \toprule
         PET & MNLI & QQP & QNLI & SST-2 & MRPC & CoLA & RTE & Average & $\Delta$\\ 
    \midrule
        \textsc{Prompt} & 34.4$_{1.2}$ & 53.2$_{5.1}$ & 51.7$_{1.7}$ & \textbf{73.3}$_{8.7}$ & 50.2$_{3.2}$ & 2.5$_{2.5}$ & 52.2$_{4.9}$ & \textbf{45.4}$_{2.1}$ &-\\
        \textsc{+Brown\_PDF} & 34.4$_{0.8}$ & 51.1$_{5.2}$ & 52.0$_{1.1}$ & 62.8$_{5.4}$ & 48.3$_{7.0}$ & 1.8$_{2.7}$ & 52.2$_{1.4}$ & 43.2$_{1.4}$ & \textbf{2.2}\\ 
        \textsc{+Brown\_SDE} & \textbf{34.5}$_{0.8}$ & \textbf{53.6}$_{6.0}$ & \textbf{52.2}$_{1.2}$ & 58.7$_{4.9}$ & \textbf{50.5}$_{10.3}$ & \textbf{2.8}$_{5.6}$ & \textbf{52.4}$_{1.8}$ & 43.5$_{1.8}$ &-1.9\\
    \midrule
        \textsc{LoRA} & 37.9$_{1.9}$ & 49.5$_{12.5}$ & 53.9$_{4.9}$ & 90.4$_{1.4}$ & 50.5$_{2.5}$ & -0.6$_{1.9}$ & 52.5$_{3.4}$ & 47.7$_{1.5}$ &-\\
        \textsc{+Brown\_PDF} & 39.6$_{3.4}$ & 54.6$_{10.7}$ & \textbf{60.2}$_{10.1}$ & \textbf{90.8}$_{1.4}$ & \textbf{54.4}$_{3.6}$ & 2.5$_{1.4}$ & 56.2$_{4.5}$ & 51.2$_{1.8}$ &3.5\\
        \textsc{+Brown\_SDE} & \textbf{40.2}$_{3.1}$ & \textbf{56.5}$_{6.0}$ & 59.9$_{7.7}$ & 89.9$_{1.5}$ & 53.9$_{4.5}$ & \textbf{11.1}$_{10.8}$ & \textbf{56.5}$_{3.2}$ & \textbf{52.6}$_{1.7}$ & \textbf{4.9}\\ 
    \midrule
        \textsc{BitFit} & 36.7$_{1.7}$ & 51.6$_{11.2}$ & 53.0$_{4.3}$ & \textbf{90.3}$_{0.6}$ & 49.0$_{7.8}$ & 3.7$_{3.1}$ & 53.8$_{2.4}$ & 48.3$_{1.6}$ &-\\
        \textsc{+Brown\_PDF} & \textbf{38.8}$_{2.8}$ & 56.6$_{7.7}$ & \textbf{57.0}$_{8.5}$ & 90.2$_{1.1}$ & 49.8$_{3.7}$ & 3.3$_{1.3}$ & \textbf{56.6}$_{3.1}$ & 50.3$_{0.6}$ &2.0\\
        \textsc{+Brown\_SDE} & 37.0$_{2.3}$ & \textbf{56.8}$_{5.7}$ & 56.5$_{7.7}$ & 86.3$_{2.1}$ & \textbf{54.8}$_{3.6}$ & \textbf{7.7}$_{4.9}$ & 56.2$_{2.6}$ & \textbf{50.8}$_{1.1}$ & \textbf{2.5}\\ 
    \midrule
        \textsc{Adapter} & 37.7$_{2.2}$ & 42.9$_{17.2}$ & 52.6$_{3.3}$ & \textbf{89.8}$_{1.0}$ & 45.4$_{8.0}$ & 5.4$_{3.1}$ & 53.6$_{4.2}$ & 46.8$_{1.9}$ &-\\
        \textsc{+Brown\_PDF} & \textbf{40.0}$_{3.5}$ & 51.8$_{12.1}$ & 54.7$_{8.2}$ & 88.1$_{2.4}$ & 47.4$_{8.1}$ & 6.9$_{1.2}$ & 55.1$_{3.6}$ & 49.1$_{2.2}$ &2.3\\
        \textsc{+Brown\_SDE} & 39.3$_{2.1}$ & \textbf{57.3}$_{9.5}$ & \textbf{60.2}$_{10.8}$ & 87.6$_{2.1}$ & \textbf{53.5}$_{5.0}$ & \textbf{11.2}$_{8.2}$ & \textbf{57.3}$_{4.6}$ & \textbf{52.3}$_{1.0}$ & \textbf{5.5}\\ 
    \bottomrule
    \end{tabular}
    \label{tab:glue-deberta-16shot}
\end{table}


==> tables/deberta_8shot.tex <==
\begin{table}[t!]
    \centering
    \caption{The results on GLUE for $\deberta$ under 8-shot setting.}
    \setlength{\tabcolsep}{4pt}
    \begin{tabular}{l *{9}{r}}
    \toprule
         PET & MNLI & QQP & QNLI & SST-2 & MRPC & CoLA & RTE & Average & $\Delta$\\ 
    \midrule
        \textsc{Prompt} & 34.4$_{1.2}$ & 53.2$_{5.1}$ & 51.7$_{1.7}$ & 73.3$_{8.7}$ & 50.2$_{3.2}$ & 2.5$_{2.5}$ & 52.2$_{4.9}$ & 45.4$_{2.1}$ &-\\
        \textsc{+Brown\_PDF} & 34.8$_{0.8}$ & 54.5$_{5.1}$ & \textbf{53.2}$_{2.2}$ & \textbf{78.4}$_{11.2}$ & \textbf{53.7}$_{3.9}$ & 3.3$_{5.1}$ & 52.9$_{2.9}$ & \textbf{47.2}$_{3.4}$ & \textbf{1.8}\\ 
        \textsc{+Brown\_SDE} & \textbf{35.6}$_{1.1}$ & \textbf{57.3}$_{4.4}$ & 52.6$_{1.2}$ & 73.9$_{13.1}$ & 52.8$_{4.0}$ & \textbf{4.5}$_{1.9}$ & \textbf{53.0}$_{2.4}$ & 47.1$_{1.7}$ &1.7\\
    \midrule
        \textsc{LoRA} & 41.0$_{1.9}$ & 56.6$_{10.3}$ & 56.3$_{4.0}$ & 90.6$_{2.4}$ & 54.9$_{1.0}$ & 4.7$_{4.4}$ & 55.0$_{3.2}$ & 51.3$_{1.1}$ &-\\
        \textsc{+Brown\_PDF} & \textbf{43.6}$_{3.3}$ & 61.3$_{8.0}$ & \textbf{68.7}$_{8.8}$ & \textbf{91.3}$_{2.6}$ & 56.3$_{3.6}$ & 8.8$_{5.0}$ & 58.7$_{3.5}$ & 55.5$_{1.3}$ &4.2\\
        \textsc{+Brown\_SDE} & 43.0$_{2.8}$ & \textbf{65.0}$_{3.5}$ & 67.1$_{8.3}$ & 89.6$_{4.1}$ & \textbf{59.1}$_{3.8}$ & \textbf{18.6}$_{14.3}$ & \textbf{60.9}$_{2.8}$ & \textbf{57.6}$_{3.1}$ & \textbf{6.3}\\ 
    \midrule
        \textsc{BitFit} & 38.2$_{1.6}$ & 57.1$_{11.2}$ & 57.0$_{4.2}$ & \textbf{90.8}$_{1.2}$ & 51.9$_{5.1}$ & 10.9$_{7.1}$ & 58.0$_{4.1}$ & 52.0$_{1.9}$ &-\\
        \textsc{+Brown\_PDF} & \textbf{41.2}$_{2.2}$ & 59.6$_{8.4}$ & 60.7$_{7.0}$ & 90.7$_{1.2}$ & 51.3$_{7.2}$ & 9.4$_{8.0}$ & \textbf{59.0}$_{3.7}$ & 53.1$_{2.6}$ &1.1\\
        \textsc{+Brown\_SDE} & 40.4$_{2.2}$ & \textbf{63.4}$_{5.3}$ & \textbf{61.8}$_{6.0}$ & 87.2$_{2.4}$ & \textbf{57.4}$_{5.5}$ & \textbf{18.1}$_{7.1}$ & 57.2$_{2.3}$ & \textbf{55.1}$_{1.5}$ & \textbf{3.1}\\ 
    \midrule
        \textsc{Adapter} & 40.2$_{2.3}$ & 58.1$_{11.0}$ & 56.8$_{3.8}$ & 89.9$_{2.7}$ & 56.7$_{2.4}$ & 11.9$_{8.2}$ & 57.1$_{4.0}$ & 53.0$_{2.0}$ &-\\
        \textsc{+Brown\_PDF} & \textbf{45.4}$_{2.9}$ & 60.5$_{9.9}$ & 64.5$_{8.3}$ & \textbf{90.9}$_{1.9}$ & 57.4$_{3.4}$ & 14.8$_{8.0}$ & 56.8$_{2.3}$ & 55.8$_{2.1}$ &2.8\\
        \textsc{+Brown\_SDE} & 42.9$_{3.5}$ & \textbf{62.9}$_{5.5}$ & \textbf{65.8}$_{9.8}$ & 89.8$_{3.1}$ & \textbf{60.7}$_{3.0}$ & \textbf{23.4}$_{5.0}$ & \textbf{57.8}$_{3.8}$ & \textbf{57.6}$_{1.7}$ & \textbf{4.6}\\ 
    \bottomrule
    \end{tabular}
    \label{tab:glue-deberta-16shot}
\end{table}


==> tables/hyperparameter_fullglue.tex <==
\begin{table}[t!]
    \centering
    % \setlength{\tabcolsep}{4.3pt}
    \caption{Hyper-parameters for training PETs on full-set GLUE.}
    \begin{tabular}{l r r}
    \toprule
        Weight decay & 0.01 \\
        Grad norm & 1.0 & \\
        Max steps & 50k & \\
        Warmup ratio & 0 \\
    \bottomrule
    \end{tabular}
    \label{tab:hyperparameter-fullglue}
\end{table}

==> tables/megatron_8_32_shot.tex <==
\begin{table}[t!]
    \centering
    \caption{Megatron 8 shot}
    \setlength{\tabcolsep}{4.3pt}
    \begin{tabular}{l *{16}{c}}
    \toprule
         PET & \multicolumn{2}{c}{MNLI} & \multicolumn{2}{c}{QQP} & \multicolumn{2}{c}{QNLI} & \multicolumn{2}{c}{SST-2} & \multicolumn{2}{c}{MRPC} & \multicolumn{2}{c}{RTE} & \multicolumn{2}{c}{Average} & \multicolumn{2}{c}{$\Delta$}\\
         \cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}\cmidrule(lr){10-11}\cmidrule(lr){12-13}\cmidrule(lr){14-15}\cmidrule(lr){16-17}
         Shot & 4 & 8 & 4 & 8 & 4 & 8 & 4 & 8 & 4 & 8 & 4 & 8 & 4 & 8 & 4 & 8 \\
    \midrule
        \textsc{Prompt} & 37.8$_{2.5}$ & 38.8$_{1.3}$ & 47.6$_{6.8}$ & 55.5$_{1.8}$ & 50.1$_{1.0}$ & 50.5$_{1.2}$ & 59.5$_{3.5}$ & 86.4$_{3.5}$ & 50.5$_{4.9}$ & 52.4$_{3.4}$ & 49.0$_{4.3}$ & 49.0$_{2.1}$ & 49.1$_{0.9}$ & 55.4$_{0.4}$&&-\\
        \textsc{+Brown\_PDF} & 38.0$_{2.2}$ & 38.8$_{1.2}$ & \textbf{54.7}$_{2.2}$ & 55.8$_{1.8}$ & 51.7$_{1.1}$ & 52.2$_{3.0}$ & 69.5$_{7.1}$ & 89.1$_{2.6}$ & 52.4$_{1.0}$ & 53.8$_{4.6}$ & 49.8$_{1.9}$ & 50.4$_{2.3}$ & 52.7$_{1.5}$ & 56.7$_{0.9}$&&1.3\\
        \textsc{+Brown\_SDE} & \textbf{38.3}$_{2.0}$ & \textbf{39.1}$_{2.0}$ & 53.4$_{3.1}$ & \textbf{56.6}$_{1.4}$ & \textbf{53.8}$_{0.4}$ & \textbf{54.9}$_{3.3}$ & \textbf{75.3}$_{11.9}$ & \textbf{89.9}$_{2.0}$ & \textbf{53.0}$_{2.7}$ & \textbf{54.7}$_{3.4}$ & \textbf{51.3}$_{0.9}$ & \textbf{52.1}$_{2.0}$ & \textbf{54.2}$_{1.7}$ & \textbf{57.9}$_{0.7}$& \textbf{5.1}& \textbf{2.5}\\
    \midrule
        \textsc{LoRA} & 48.5$_{2.2}$ & 55.2$_{1.9}$ & 56.8$_{4.8}$ & 66.2$_{1.6}$ & 51.1$_{2.4}$ & 60.9$_{4.2}$ & 90.5$_{0.8}$ & 91.0$_{0.6}$ & 51.0$_{3.8}$ & 57.4$_{4.0}$ & 62.7$_{2.7}$ & 64.3$_{2.7}$ & 60.1$_{1.1}$ & 65.8$_{1.2}$&&-\\
        \textsc{+Brown\_PDF} & 49.5$_{2.9}$ & 57.3$_{2.9}$ & 58.9$_{5.5}$ & 67.5$_{1.9}$ & 52.6$_{3.1}$ & 63.6$_{3.7}$ & \textbf{90.6}$_{0.8}$ & \textbf{91.2}$_{0.2}$ & 52.2$_{4.3}$ & 60.8$_{3.6}$ & 64.2$_{2.2}$ & 64.8$_{1.2}$ & 61.3$_{1.4}$ & 67.5$_{0.7}$&&1.7\\
        \textsc{+Brown\_SDE} & \textbf{51.1}$_{1.3}$ & \textbf{61.1}$_{1.2}$ & \textbf{59.7}$_{3.5}$ & \textbf{68.1}$_{1.1}$ & \textbf{62.0}$_{5.1}$ & \textbf{68.2}$_{5.2}$ & 90.5$_{0.4}$ & \textbf{91.2}$_{0.2}$ & \textbf{56.5}$_{5.5}$ & \textbf{62.6}$_{3.2}$ & \textbf{64.4}$_{1.3}$ & \textbf{65.3}$_{0.5}$ & \textbf{64.0}$_{1.2}$ & \textbf{69.4}$_{0.5}$& \textbf{3.9}& \textbf{3.6}\\
    \midrule
        \textsc{BitFit} & 48.5$_{2.6}$ & 52.3$_{1.5}$ & 52.0$_{4.8}$ & 60.6$_{1.4}$ & 49.9$_{2.1}$ & 53.7$_{1.7}$ & 88.0$_{2.9}$ & 90.9$_{0.3}$ & 50.8$_{3.9}$ & 52.6$_{2.3}$ & 58.4$_{6.1}$ & 63.7$_{0.7}$ & 57.9$_{1.6}$ & 62.3$_{0.7}$&&-\\
        \textsc{+Brown\_PDF} & 49.1$_{2.6}$ & 53.3$_{1.2}$ & 52.1$_{5.0}$ & 62.0$_{2.7}$ & 50.5$_{2.5}$ & 55.9$_{0.9}$ & \textbf{90.5}$_{0.8}$ & \textbf{91.0}$_{0.5}$ & 50.8$_{2.2}$ & 54.3$_{1.9}$ & 61.0$_{3.8}$ & 63.8$_{2.2}$ & 59.0$_{1.1}$ & 63.4$_{0.5}$&&1.1\\
        \textsc{+Brown\_SDE} & \textbf{49.5}$_{2.1}$ & \textbf{54.5}$_{1.3}$ & \textbf{55.5}$_{4.0}$ & \textbf{65.5}$_{2.2}$ & \textbf{57.1}$_{2.6}$ & \textbf{63.5}$_{4.5}$ & 90.4$_{0.4}$ & 90.9$_{0.3}$ & \textbf{53.4}$_{3.2}$ & \textbf{58.2}$_{2.0}$ & \textbf{63.8}$_{1.3}$ & \textbf{64.3}$_{2.5}$ & \textbf{61.6}$_{1.2}$ & \textbf{66.1}$_{0.7}$& \textbf{3.7}& \textbf{3.8}\\ 
    \midrule
        \textsc{Adapter} & 47.1$_{3.0}$ & 54.2$_{1.7}$ & 54.1$_{4.5}$ & 64.6$_{3.0}$ & 53.0$_{2.6}$ & 59.5$_{1.9}$ & 89.2$_{3.6}$ & 91.5$_{0.3}$ & 50.3$_{4.7}$ & 59.4$_{2.5}$ & 60.8$_{3.6}$ & 62.9$_{3.1}$ & 59.1$_{1.8}$ & 65.3$_{0.6}$&&-\\
        \textsc{+Brown\_PDF} & 48.0$_{3.3}$ & 56.4$_{2.2}$ & 56.3$_{4.4}$ & 66.9$_{1.4}$ & 54.5$_{3.4}$ & 63.5$_{3.1}$ & 89.4$_{3.8}$ & \textbf{91.8}$_{0.3}$ & 52.0$_{5.7}$ & 61.1$_{2.7}$ & 61.7$_{3.3}$ & 63.8$_{2.2}$ & 60.3$_{1.9}$ & 67.3$_{0.6}$&&2.0\\
        \textsc{+Brown\_SDE} & \textbf{50.0}$_{2.5}$ & \textbf{58.9}$_{1.1}$ & \textbf{58.1}$_{2.9}$ & \textbf{69.3}$_{1.6}$ & \textbf{59.8}$_{4.7}$ & \textbf{70.1}$_{5.1}$ & \textbf{91.1}$_{0.9}$ & 91.7$_{0.4}$ & \textbf{53.5}$_{6.1}$ & \textbf{61.6}$_{2.5}$ & \textbf{62.6}$_{3.5}$ & \textbf{64.4}$_{0.9}$ & \textbf{62.5}$_{1.8}$ & \textbf{69.3}$_{0.6}$& \textbf{3.4}& \textbf{4.0}\\

    \bottomrule
    \end{tabular}
    \label{tab:my_label}
\end{table}

==> tables/megatron_glue_fewshot_32shot.tex <==
\begin{table}[t!]
    \centering
    \caption{The results on GLUE for $\megatronbert$ under 32-shot setting.}
    % \setlength{\tabcolsep}{5pt}
    \begin{tabular}{l *{8}{r}}
    \toprule
         PET & MNLI & QQP & QNLI & SST-2 & MRPC & RTE & Average & $\Delta$\\ 
    \midrule
        \textsc{Prompt} & 38.8$_{1.3}$ & 55.5$_{1.8}$ & 50.5$_{1.2}$ & 86.4$_{3.5}$ & 52.4$_{3.4}$ & 49.0$_{2.1}$ & 55.4$_{0.4}$ &-\\
        \textsc{+Brown\_PDF} & 38.8$_{1.2}$ & 55.8$_{1.8}$ & 52.2$_{3.0}$ & 89.1$_{2.6}$ & 53.8$_{4.6}$ & 50.6$_{3.3}$ & 56.7$_{1.0}$ &1.3\\
        \textsc{+Brown\_SDE} & 39.1$_{2.0}$ & 56.6$_{1.4}$ & 54.9$_{3.3}$ & 89.9$_{2.0}$ & 54.7$_{3.4}$ & 52.1$_{2.0}$ & 57.9$_{0.7}$ &2.5\\
    \midrule
        \textsc{LoRA} & \textbf{55.2}$_{1.9}$ & \textbf{66.2}$_{1.6}$ & \textbf{60.9}$_{4.2}$ & \textbf{91.0}$_{0.6}$ & \textbf{57.4}$_{4.0}$ & \textbf{64.3}$_{2.7}$ & \textbf{65.8}$_{1.2}$ & \textbf{10.4}\\ 
        \textsc{+Brown\_PDF} & 57.3$_{2.9}$ & 67.5$_{1.9}$ & 63.6$_{3.7}$ & 91.2$_{0.2}$ & 60.8$_{3.6}$ & 64.8$_{1.2}$ & 67.5$_{0.7}$ &nan\\
        \textsc{+Brown\_SDE} & \textbf{61.1}$_{1.2}$ & \textbf{68.1}$_{1.1}$ & \textbf{68.2}$_{5.2}$ & \textbf{91.2}$_{0.2}$ & \textbf{62.6}$_{3.2}$ & \textbf{65.3}$_{0.5}$ & \textbf{69.4}$_{0.5}$ &-\\
    \midrule
        \textsc{BitFit} & 52.3$_{1.5}$ & 60.6$_{1.4}$ & 53.7$_{1.7}$ & 90.9$_{0.3}$ & 52.6$_{2.3}$ & 63.7$_{0.7}$ & 62.3$_{0.7}$ & \textbf{7.1}\\ 
        \textsc{+Brown\_PDF} & 53.3$_{1.2}$ & 62.0$_{2.7}$ & 55.9$_{0.9}$ & 91.0$_{0.5}$ & 54.3$_{1.9}$ & 63.8$_{2.2}$ & 63.4$_{0.5}$ &-6.0\\
        \textsc{+Brown\_SDE} & 54.5$_{1.3}$ & 65.5$_{2.2}$ & 63.5$_{4.5}$ & 90.9$_{0.3}$ & 58.2$_{2.0}$ & 64.3$_{2.5}$ & 66.1$_{0.7}$ &-3.3\\
    \midrule
        \textsc{Adapter} & 54.2$_{1.7}$ & 64.6$_{3.0}$ & 59.5$_{1.9}$ & 91.5$_{0.3}$ & 59.4$_{2.5}$ & 62.9$_{3.1}$ & 65.3$_{0.6}$ &-\\
        \textsc{+Brown\_PDF} & 56.4$_{2.2}$ & 66.9$_{1.4}$ & 63.5$_{3.1}$ & \textbf{91.8}$_{0.3}$ & 61.1$_{2.7}$ & 63.8$_{2.2}$ & 67.3$_{0.6}$ &2.0\\
        \textsc{+Brown\_SDE} & \textbf{58.9}$_{1.1}$ & \textbf{69.3}$_{1.6}$ & \textbf{70.1}$_{5.1}$ & 91.7$_{0.4}$ & \textbf{61.6}$_{2.5}$ & \textbf{64.4}$_{0.9}$ & \textbf{69.3}$_{0.6}$ & \textbf{4.0}\\ 
    \bottomrule
    \end{tabular}
    \label{tab:glue-4shot}
\end{table}

==> tables/megatron_glue_fewshot_4shot.tex <==
\begin{table}[t!]
    \centering
    \caption{The results on GLUE for $\megatronbert$ under 4-shot setting.}
    % \setlength{\tabcolsep}{5pt}
    \begin{tabular}{l *{8}{r}}
    \toprule
         PET & MNLI & QQP & QNLI & SST-2 & MRPC & RTE & Average & $\Delta$\\ 
    \midrule
        \textsc{Prompt} & 36.8$_{1.1}$ & 45.9$_{5.1}$ & 50.6$_{1.4}$ & 56.4$_{5.7}$ & 51.1$_{1.2}$ & 47.6$_{3.6}$ & 48.1$_{0.5}$ &-\\
        \textsc{+Brown\_PDF} & 37.2$_{2.8}$ & 50.6$_{5.6}$ & 51.6$_{1.5}$ & 63.3$_{10.6}$ & \textbf{54.6}$_{2.9}$ & 49.5$_{3.2}$ & 51.1$_{1.7}$ &3.0\\
        \textsc{+Brown\_SDE} & 37.7$_{2.4}$ & 52.4$_{4.4}$ & \textbf{52.1}$_{1.3}$ & 71.4$_{7.5}$ & 52.1$_{2.4}$ & 52.4$_{1.1}$ & 53.0$_{1.6}$ &4.9\\
    \midrule
        \textsc{LoRA} & \textbf{47.7}$_{3.1}$ & \textbf{52.6}$_{4.2}$ & 50.4$_{1.1}$ & \textbf{89.3}$_{2.4}$ & 50.1$_{2.5}$ & \textbf{58.3}$_{3.5}$ & \textbf{58.1}$_{1.3}$ & \textbf{10.0}\\ 
        \textsc{+Brown\_PDF} & 48.5$_{4.0}$ & 55.8$_{4.5}$ & 52.6$_{3.7}$ & 89.2$_{2.4}$ & 51.2$_{4.1}$ & 59.6$_{3.4}$ & 59.5$_{1.3}$ &nan\\
        \textsc{+Brown\_SDE} & 48.2$_{3.5}$ & \textbf{54.4}$_{3.6}$ & \textbf{57.5}$_{5.4}$ & \textbf{89.2}$_{2.4}$ & \textbf{52.6}$_{7.3}$ & \textbf{61.8}$_{1.2}$ & \textbf{60.6}$_{1.8}$ &-\\
    \midrule
        \textsc{BitFit} & 46.9$_{3.1}$ & 50.3$_{4.8}$ & 49.7$_{2.2}$ & 86.3$_{2.6}$ & 49.5$_{3.6}$ & 55.8$_{3.6}$ & 56.4$_{1.0}$ & \textbf{4.2}\\ 
        \textsc{+Brown\_PDF} & 48.8$_{2.6}$ & 50.2$_{4.9}$ & 50.4$_{2.4}$ & 88.2$_{2.5}$ & 50.4$_{3.0}$ & 56.8$_{4.4}$ & 57.5$_{1.6}$ &-3.1\\
        \textsc{+Brown\_SDE} & \textbf{49.0}$_{2.6}$ & 51.4$_{4.7}$ & 53.7$_{2.5}$ & 88.9$_{1.2}$ & 49.7$_{3.0}$ & 59.3$_{0.5}$ & 58.7$_{1.6}$ &-1.9\\
    \midrule
        \textsc{Adapter} & 45.0$_{3.4}$ & 50.4$_{4.9}$ & 52.0$_{3.2}$ & 87.7$_{1.8}$ & 49.8$_{3.6}$ & 56.8$_{3.9}$ & 57.0$_{1.5}$ &-\\
        \textsc{+Brown\_PDF} & \textbf{47.1}$_{3.6}$ & 51.9$_{6.4}$ & 53.4$_{5.2}$ & 89.1$_{1.9}$ & 52.9$_{5.9}$ & 58.1$_{6.0}$ & 58.7$_{1.1}$ &1.7\\
        \textsc{+Brown\_SDE} & 46.9$_{3.2}$ & \textbf{52.0}$_{7.5}$ & \textbf{57.6}$_{3.7}$ & \textbf{90.4}$_{1.8}$ & \textbf{53.3}$_{3.7}$ & \textbf{60.5}$_{3.9}$ & \textbf{60.1}$_{1.8}$ & \textbf{3.1}\\ 
    \bottomrule
    \end{tabular}
    \label{tab:glue-4shot}
\end{table}

==> tables/megatron_glue_fewshot_8shot.tex <==
\begin{table}[t!]
    \centering
    \caption{The results on GLUE for $\megatronbert$ under 8-shot setting.}
    % \setlength{\tabcolsep}{5pt}
    \begin{tabular}{l *{8}{r}}
    \toprule
         PET & MNLI & QQP & QNLI & SST-2 & MRPC & RTE & Average & $\Delta$\\ 
    \midrule
        \textsc{Prompt} & 37.8$_{2.5}$ & 47.6$_{6.8}$ & 50.1$_{1.0}$ & 59.5$_{3.5}$ & 50.5$_{4.9}$ & 49.0$_{4.3}$ & 49.1$_{0.9}$ &-\\
        \textsc{+Brown\_PDF} & 38.0$_{2.2}$ & 54.7$_{2.2}$ & 51.7$_{1.1}$ & 69.5$_{7.1}$ & 52.4$_{1.0}$ & 49.8$_{1.9}$ & 52.7$_{1.5}$ &3.6\\
        \textsc{+Brown\_SDE} & 38.3$_{2.0}$ & 53.4$_{3.1}$ & \textbf{53.8}$_{0.4}$ & 75.3$_{11.9}$ & \textbf{53.0}$_{2.7}$ & 51.3$_{0.9}$ & 54.2$_{1.7}$ &5.1\\
    \midrule
        \textsc{LoRA} & \textbf{48.5}$_{2.2}$ & \textbf{56.8}$_{4.8}$ & 51.1$_{2.4}$ & \textbf{90.5}$_{0.8}$ & 51.0$_{3.8}$ & \textbf{62.7}$_{2.7}$ & \textbf{60.1}$_{1.1}$ & \textbf{11.0}\\ 
        \textsc{+Brown\_PDF} & 49.5$_{2.9}$ & 58.9$_{5.5}$ & 52.6$_{3.1}$ & 90.6$_{0.8}$ & 52.2$_{4.3}$ & 64.2$_{2.2}$ & 61.3$_{1.4}$ &nan\\
        \textsc{+Brown\_SDE} & \textbf{51.1}$_{1.3}$ & \textbf{59.7}$_{3.5}$ & \textbf{62.0}$_{5.1}$ & \textbf{90.5}$_{0.4}$ & \textbf{56.5}$_{5.5}$ & \textbf{64.4}$_{1.3}$ & \textbf{64.0}$_{1.2}$ &-\\
    \midrule
        \textsc{BitFit} & 48.5$_{2.6}$ & 52.0$_{4.8}$ & 49.9$_{2.1}$ & 88.0$_{2.9}$ & 50.8$_{3.9}$ & 58.4$_{6.1}$ & 57.9$_{1.6}$ & \textbf{6.1}\\ 
        \textsc{+Brown\_PDF} & 49.1$_{2.6}$ & 52.1$_{5.0}$ & 50.5$_{2.5}$ & \textbf{90.5}$_{0.8}$ & 50.8$_{2.2}$ & 61.0$_{3.8}$ & 59.0$_{1.1}$ &-5.0\\
        \textsc{+Brown\_SDE} & 49.5$_{2.1}$ & 55.5$_{4.0}$ & 57.1$_{2.6}$ & 90.4$_{0.4}$ & 53.4$_{3.2}$ & 63.8$_{1.3}$ & 61.6$_{1.2}$ &-2.4\\
    \midrule
        \textsc{Adapter} & 47.1$_{3.0}$ & 54.1$_{4.5}$ & 53.0$_{2.6}$ & 89.2$_{3.6}$ & 50.3$_{4.7}$ & 60.8$_{3.6}$ & 59.1$_{1.8}$ &-\\
        \textsc{+Brown\_PDF} & 48.0$_{3.3}$ & 56.3$_{4.4}$ & 54.5$_{3.4}$ & 89.4$_{3.8}$ & 52.0$_{5.7}$ & 61.7$_{3.3}$ & 60.3$_{1.9}$ &1.2\\
        \textsc{+Brown\_SDE} & \textbf{50.0}$_{2.5}$ & \textbf{58.1}$_{2.9}$ & \textbf{59.8}$_{4.7}$ & \textbf{91.1}$_{0.9}$ & \textbf{53.5}$_{6.1}$ & \textbf{62.6}$_{3.5}$ & \textbf{62.5}$_{1.8}$ & \textbf{3.4}\\ 
    \bottomrule
    \end{tabular}
    \label{tab:glue-4shot}
\end{table}

==> tables/ou_glue_full.tex <==

\begin{table}[t!]
    \centering
    \begin{tabular}{l c c c c c c c c}
        \toprule
            & MNLI & QQP & QNLI & SST-2 & MRPC & CoLA & RTE & Average\\
            \midrule
            \textsc{Prompt} & 84.4$_{0.1}$ & 85.3$_{0.3}$ & 91.5$_{0.1}$ & 95.5$_{0.1}$ & 73.9$_{2.4}$ & 55.5$_{3.4}$ & 60.8$_{1.5}$ & 78.1$_{0.6}$\\
            \textsc{+OU\_PDF} & 84.7$_{0.1}$ & 85.4$_{0.1}$ & 91.8$_{0.3}$ & 95.6$_{0.2}$ & 76.9$_{1.0}$ & 57.1$_{1.2}$ & 60.5$_{3.0}$ & 78.9$_{0.2}$\\
            \textsc{+OU\_SDE} & 84.7$_{0.2}$ & 85.3$_{0.1}$ & 92.1$_{0.3}$ & 95.5$_{0.2}$ & 80.2$_{0.5}$ & 61.5$_{3.5}$ & 65.9$_{2.7}$ & 80.7$_{0.8}$\\
        \midrule
            \textsc{LoRA} & 88.8$_{0.1}$ & 89.2$_{0.2}$ & 93.5$_{0.2}$ & 95.5$_{0.1}$ & 84.6$_{0.4}$ & 62.8$_{1.6}$ & 78.9$_{1.6}$ & 84.8$_{0.3}$\\
            \textsc{+OU\_PDF} & 88.9$_{0.2}$ & 89.4$_{0.1}$ & 93.7$_{0.1}$ & 95.7$_{0.3}$ & 86.0$_{0.5}$ & 63.6$_{0.6}$ & 80.5$_{0.8}$ & 85.4$_{0.1}$\\
            \textsc{+OU\_SDE} & 88.8$_{0.0}$ & 89.5$_{0.1}$ & 93.7$_{0.2}$ & 95.7$_{0.3}$ & 86.3$_{1.2}$ & 63.7$_{0.6}$ & 80.1$_{0.9}$ & 85.4$_{0.1}$\\
        \midrule
            \textsc{BitFit} & 87.9$_{0.2}$ & 87.6$_{0.1}$ & 92.7$_{0.2}$ & 95.6$_{0.1}$ & 79.4$_{2.3}$ & 60.2$_{0.8}$ & 77.0$_{1.5}$ & 82.9$_{0.3}$\\
            \textsc{+OU\_PDF} & 87.9$_{0.1}$ & 87.8$_{0.1}$ & 93.0$_{0.1}$ & 95.7$_{0.1}$ & 82.6$_{0.8}$ & 59.8$_{1.0}$ & 78.8$_{1.4}$ & 83.6$_{0.4}$\\
            \textsc{+OU\_SDE} & 87.9$_{0.1}$ & 87.6$_{0.1}$ & 92.7$_{0.1}$ & 95.8$_{0.1}$ & 83.7$_{0.8}$ & 60.8$_{1.6}$ & 77.1$_{0.9}$ & 83.7$_{0.4}$\\
        \midrule
            \textsc{Adapter} & 88.8$_{0.1}$ & 89.6$_{0.3}$ & 93.7$_{0.1}$ & 95.6$_{0.1}$ & 83.6$_{0.1}$ & 60.4$_{1.2}$ & 79.5$_{1.2}$ & 84.5$_{0.3}$\\
            \textsc{+OU\_PDF} & 88.9$_{0.1}$ & 89.7$_{0.0}$ & 93.8$_{0.1}$ & 95.8$_{0.1}$ & 86.8$_{0.6}$ & 61.9$_{0.2}$ & 82.0$_{0.6}$ & 85.6$_{0.1}$\\
            \textsc{+OU\_SDE} & 88.9$_{0.1}$ & 89.8$_{0.1}$ & 93.7$_{0.1}$ & 95.7$_{0.1}$ & 85.9$_{0.7}$ & 62.5$_{1.2}$ & 82.7$_{0.5}$ & 85.6$_{0.2}$\\
        \bottomrule
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}

==> tables/perf_bridgeloss.tex <==
\begin{wraptable}{r}{4.0cm}
    \centering
    % \vspace{-0.4em}
    \caption{Pearson's correlation between the performance and the distance to the latent bridges.}
    % \vspace{-0.5em}
    \label{tab:perf-bridgeloss}
    \small
    \begin{tabular}{l r@{}l r@{}l}
        \toprule
        Dataset & \multicolumn{2}{c}{Coef.} & \multicolumn{2}{c}{$\mathit{p}$-value} \\
        \midrule
        MNLI & -0&.09 & .715& \\
        QQP & -0&.42 & .062& \\
        QNLI & -0&.77 & $<$.001&$^{***}$ \\
        SST-2 & -0&.69 & $<$.001&$^{***}$ \\
        MRPC & -0&.13 & .591& \\
        RTE & -0&.87 & $<$.001&$^{***}$ \\
    \bottomrule
    \end{tabular}
    \vspace{-2em}
\end{wraptable}

==> tables/shot_bridgeloss.tex <==
\begin{wraptable}{r}{4.0cm}
    \centering
    \vspace{-1.5em}
    \caption{Kendall's rank correlation between the number of shots and the distance to the latent bridges.}
    \vspace{-1em}
    \label{tab:shot-bridgeloss}
    \small
    \begin{tabular}{l r@{}l r@{}l}
        \toprule
        Dataset & \multicolumn{2}{c}{Coef.} & \multicolumn{2}{c}{$\mathit{p}$-value} \\
        \midrule
        MNLI & -0&.39 & .026&$^{*}$ \\
        QQP & -0&.36 & .037&$^{*}$ \\
        QNLI & -0&.32 & .069& \\
        SST-2 & -0&.50 & .005&$^{**}$ \\
        MRPC & -0&.21 & .225& \\
        RTE & -0&.34 & .049&$^{*}$ \\
    \bottomrule
    \end{tabular}
    \vspace{-3em}
\end{wraptable}
